Public repository with Monte Carlo simulations for high-energy particle collision experiments

Planning high-energy collision experiments for the next few decades requires extensive Monte Carlo simulations in order to accomplish physics goals of these experiments. Such simulations are essential for understanding fundamental physics processes, as well as for setting up the detector parameters that help establish R&D projects required over the next few decades. This paper describes a public repository with Monte Carlo event samples before and after detector-response simulation. The goal of this repository is to facilitate the accomplishment of many goals in planning a next generation of particle experiments.

==> Makefile <==
NOTENAME = ichep16
TEX := latex

.PHONY: all clean

all:#default target makes everything
	$(TEX) $(NOTENAME).tex
	$(TEX) $(NOTENAME).tex
	dvips -Ppdf -G0  $(NOTENAME).dvi
	ps2pdf $(NOTENAME).ps $(NOTENAME).pdf
 
show:
	evince $(NOTENAME).pdf

clean:
	rm -rf $(NOTENAME).aux $(NOTENAME).log $(NOTENAME).out $(NOTENAME).bbl $(NOTENAME).blg \
	$(NOTENAME).dvi $(NOTENAME).ps \
	$(NOTENAME).toc $(NOTENAME).tof thumb*.* $(NOTENAME).pdf

